A Fine-Grained Hybrid CPU-GPU Algorithm for Betweenness Centrality Computations

Betweenness centrality (BC) is an important graph analytical application for large-scale graphs. While there are many efforts for parallelizing betweenness centrality algorithms on multi-core CPUs and many-core GPUs, in this work, we propose a novel fine-grained CPU-GPU hybrid algorithm that partitions a graph into CPU and GPU partitions, and performs BC computations for the graph on both the CPU and GPU resources simultaneously with very small number of CPU-GPU communications. The forward phase in our hybrid BC algorithm leverages the multi-source property inherent in the BC problem. We also perform a novel hybrid and asynchronous backward phase that performs minimal CPU-GPU synchronizations. Evaluations using a large number of graphs with different characteristics show that our hybrid approach gives 80% improvement in performance, and 80-90% less CPU-GPU communications than an existing hybrid algorithm based on the popular Bulk Synchronous Paradigm (BSP) approach.

==> results.tex <==
Need to show:
idling or utilization results
backward phase results. (naive vs ours)
exploring large graphs
naive vs our partioning
multiple gpu

Sariyuce:
Since the computations can be extremely long (months), we measured the time for a given number of sources/BFSs and extrapolated linearly to the runtime for all the graph, paying attention to take properly into account the constant one-time overheads of the application. Depending on the speed of the configuration, we run one thousand, ten thousand, or hundred thousand sources which provide a runtime large enough to smoothen any system fluctuations. The runtime of single source proved to be very stable, allowing us to make a meaningful extrapolation.
Reporting in times
Also in teps: V*E/runtime

Madduri-ipdps09:
random 256
reporting in teps using eq1 formula. (7n etc.)

McGlaughlin:
exact bc for all vertices. they consider a max of 1 million.
teps = mn/t

Pingali and Prountzos:
For large-scale graphs, it is computationally infeasible to compute BC by doing shortest path computations from every node of
the graph. Therefore, like previous studies [4,16,19,29], we perform shortest path computations for only a subset of nodes.

Sariyuce. Regularizing. JPDC 2015:
Since the computations can be extremely long (months), we did not used all the n BFS sources in the graphs and measured the time for 1024 sources/BFSs in total. We observed that the runtimes of single kernel executions to be very stable, allowing us to make a meaningful extrapolation. Thus, if necessary, the results can be used to linearly extrapolate the runtime for the whole graph.
TEPS = mxk/time

So:
TEPS = mxk/time or MTEPS.
Based on time available and time taken for single root with all algorithms.
Minimum = 1024.

